Actor-Context-Actor Relation Network for Spatio-Temporal Action Localization

Localizing persons and recognizing their actions from videos is a challenging task towards high-level video understanding. Recent advances have been achieved by modeling direct pairwise relations between entities. In this paper, we take one step further, not only model direct relations between pairs but also take into account indirect higher-order relations established upon multiple elements. We propose to explicitly model the Actor-Context-Actor Relation, which is the relation between two actors based on their interactions with the context. To this end, we design an Actor-Context-Actor Relation Network (ACAR-Net) which builds upon a novel High-order Relation Reasoning Operator and an Actor-Context Feature Bank to enable indirect relation reasoning for spatio-temporal action localization. Experiments on AVA and UCF101-24 datasets show the advantages of modeling actor-context-actor relations, and visualization of attention maps further verifies that our model is capable of finding relevant higher-order relations to support action detection. Notably, our method ranks first in the AVA-Kineticsaction localization task of ActivityNet Challenge 2020, out-performing other entries by a significant margin (+6.71mAP). Training code and models will be available at https://github.com/Siyu-C/ACAR-Net.

==> 01-Introduction.tex <==
\section{Introduction}
\label{sec:intro}

% \zs{as shown in Fig. 1, to detect the action of ride performed by the person in red}
% 
%Consider Fig.~\ref{fig:figure1}: the action ``ride" that is performed by the actor in the red bounding box. 
Spatio-temporal action localization, requiring localizing persons while recognizing their actions, is an important task that has drawn increasing attention in recent years \cite{gu2018ava, girdhar2019video, feichtenhofer2019slowfast, wu2019long, sun2018actor}. Unlike object detection which can be accomplished solely by observing visual appearances, activity recognition usually demands for reasoning about the actor’s interactions with the surrounding context, including other people and objects. Take Fig.~\ref{fig:figure1} as an example: to recognize the action ``ride'' of the person in the red bounding box, we need to observe that he is inside a car, and there is a driver next to him. Therefore, recent progresses in spatio-temporal action detection have been driven by the success of relation modeling. Such attempts on relation modeling can be categorized into two types:

(1) \textbf{Modeling relation between actors} \cite{girdhar2019video, wu2019long} focuses on interactions between persons, \textit{e.g.} the relation between the actor in the red bounding box (red actor) and the other in the blue bounding box (blue actor) in Fig.~\ref{fig:figure1}. These methods take feature vectors extracted from cropped actor bounding boxes as inputs. They utilize attention mechanisms to directly infer relations between actor features. 
%\sout{The success of Action Transformer \cite{girdhar2019video} and Long-term Feature Bank (LFB) \cite{wu2019long} has demonstrated the superiority of action-action relation reasoning over vanilla classifiers.} 
However, this type of methods only use information within cropped boxes, and discard important contextual information, such as spatio-temporal locations as well as contextual objects' dynamics and appearances that are helpful for more accurate reasoning.
%\zs{might be too detailed to incorporate terms like ROI}

\begin{figure*}[!t]
\centering
\includegraphics[width=\textwidth]{fig/figure_1_app.pdf}
\caption{Reasoning actor-context or actor-actor relations may not be sufficient for correctly predicting the action labels of all individuals. Our method does not only reason relations between actors, but also model connections between different actor-context relations. As an example, the relation between the blue actor and the steering wheel (drive) serves as a crucial clue for recognizing the action being performed by the red actor (ride). \label{fig:figure1}
% \zs{add red blue color box edge to cropped person as well. left image may not need color filling, just bold edge is good I think}%\zs{need highlight action class of red person in figure; caption changes to \{actor,context\} (e.g. ACRN) \{actor,actor\} (e.g. FBO)} \{actor,context, actor\}. somehow add some arrows/line to show relation.
% \pan{boxes added! fillings are more transparent now.}
}
\vspace{-4mm}
\end{figure*}

(2) \textbf{Modeling relation between actor and context} \cite{sun2018actor}, 
% \zs{In Fig. 1, this approach can identify the spatial regions (e.g. steering wheel) that are highly correlated with with the actor (e.g. person with blue box)} 
on the other hand, leverages spatio-temporal context for recognizing the behavior of an actor. As shown in Fig.~\ref{fig:figure1}, it performs relation reasoning by identifying spatial regions (\textit{e.g.} steering wheel) that have highest correlation with the blue actor to recognize his action. This type of methods do not explicitly model the relationship among actors. 
%\sout{They perform relation reasoning by identifying spatial regions that have highest correlation with each actor}. 
The advantage of these methods is that they preserve structural information which could be important for understanding the entire scene.

However, these two attempts will struggle on recognizing the action ``ride'' being performed by the red actor, since neither of these relations (actor-actor or actor-context) can provide sufficient clues. More concretely, in Fig.~\ref{fig:figure1}, it is difficult to infer the action of the red actor solely given its relation with the blue actor or with the scene context (steering wheel). To overcome this problem, we propose to capture the implicit \textit{high-order} relation between the two actors based on their respective \textit{first-order} relations with the context. In this way, we will be able to identify the action (ride) of red actor by reasoning over the interaction between the blue actor and the context (drive).
% \zs{--> indirect?}
% Motivation, explain with an example
% However, these two attempts focus only on modeling the first-order \zs{--> direct? } actor-actor or actor-context relations, which often might not be enough to correctly classify actions. 
%\zs{cannot detect xxx in Fig. 1. because xxx}
% \zs{to overcome this challenge, we propose to xx (intuition level)}
% Thus in such an example, a good algorithm should be able to capture the implicit high-order\zs{--> indirect?} relation between the two actors based on their respective interactions with the context.

% Introduce our method with some details, advantage.
% \zs{explain at the approach level. make it better structured if possible. (1) (2) (3) }

Given the need for high-order relation reasoning to understand videos, we propose an Actor-Context-Actor Relation Network (ACAR-Net) that deduces indirect relations between multiple actors and the context while being trained on the action localization task. The ACAR-Net takes both actor and context features as inputs. It first encodes the \textit{first-order actor-context} relations, and then applies a \textbf{High-Order Relation Reasoning Operator} in charge of modeling links established on those first-order relations. Finally, to model long-term high-order relations, we build an \textbf{Actor-Context Feature Bank}, which contains actor-context relations at different time stamps across the whole video.
% \zs{I'd suggest rethinking the name; multi-actor sounds like actor-actor-actor, does not include object context.}


% The network takes both actor and context features as inputs. It first capture interaction between actors and context and then reason over these interactions obtaining high-order relational feature. Specifically, both actor-context interaction and high-order relation is computed for each spatial location independently, thus the model not only can leverage semantic information but also geometric ones. To this end, the network blends structured reasoning with attention mechanisms, that can perform reasoning over large set of entities while preserving the overall structure of the scene.
% \pan{maybe no need to mention the specific attention module but only give a general concept of what it is doing}
% GIVE THE OBJECTIVE OF ATTENTION INSTEAD OF DETAILED OPERATIONS. JUST ATTENTION SOUNDS SIMPLE, GIVE IT SOME DESCRIPTIVE WORDS. The XXX attention mechanism is efficiently expressed with convolutions where the size of the kernel can be choose depending on how much neighbouring information want to use. 
% Our proposed ACAR-Net is a versatile and extensible module, which can be plug-and-play into any existing video frameworks and is compatible with the recently introduced long-term feature banks.

%What we expect with MARN
ACAR-Net learns to reason high-order relations among actors and the context, while preserving the spatial structure of the scene. Partly similar to our approach, there exist works that explicitly model interactions between actors and objects~\cite{wang2018videos, zhang2019structured}. However, in these approaches, when deducing the action of one person, the interactions of other persons with contextual objects are ignored. In other words, they do not explicitly model the higher-order relations built on direct actor-context relations. In contrast, our method emphasizes modeling those indirect relations, and does not need the extra step of object detection.
% , and also require an extra step of object detection
%These factors turn out to be the keys for correctly understanding human actions in complex scenes.
% and also provides additional feedback for learning better first-order relationships. ANY EXPERIMENT TO DEMONSTRATE THE CLAIM? IF NOT, BE CAREFUL. \pan{need to verify with the mAP of HHI and HOI} 

We conduct extensive experiments on the challenging Atomic Visual Actions (AVA) dataset~\cite{gu2018ava} for spatio-temporal action localization. This dataset contains a large number of complex realistic scenes, and most of its action classes are human-object or human-human interactions.
% For this reason it becomes the ideal tested for our approach. 
We show that our proposed ACAR-Net provides a clear advantage over previous methods on this benchmark.

% Our contributions can be summarized as three-fold: (a) To model the complex high-order relations between actors and context, we propose a novel high-order relation reasoning module for improving spatial-temporal action localization; (b) USE COMPLETE SENTENCES FOR CONTRIBUTIONS. We present an attention operator in forms of convolutions which is locally in space and time, non-local across actors); (c) We achieve state-of-the-art performance with significant margins on the challenging AVA dataset for spatio-temporal localization.
% \pan{Maybe just remind the major contribution}
% \zs{list contributions in bullets. can move some innovative claims above to here 1. idea/intuition ACA such an important factor for action detection 2. a novel model 3. state-of-the-art results}
Our contributions are summarized as the following: 
\begin{itemize}
\item We propose to model high-order actor-context-actor relations for spatio-temporal action localization. Such relations are mostly ignored by previous methods but crucial for achieving accurate action localization.
% \item We introduce the concept of modeling high-order relation in videos which is an important factor for action detection.
\item We propose a novel Actor-Context-Actor Relation Network for improving spatio-temporal action localization by explicitly reasoning about high-order relations between actors and the context.
\item We achieve state-of-the-art performances with significant margins on the AVA dataset.
\end{itemize}

% The major contribution of this work is that we propose a novel high-order relation reasoning module that is able to learn from  complex high-order relations between actors and context, and as result it significantly improves spatial-temporal action localization performances on the challenging AVA dataset.
